A Comprehensive Review of Lunar-based Manufacturing and Construction

As humankind prepares to establish outposts and infrastructure on the Moon, the ability to manufacture parts and buildings on-site is crucial. While transporting raw materials from Earth can be costly and time-consuming, in-situ resource utilization (ISRU) presents an attractive alternative. This review paper aims to provide a thorough examination of the current state and future potential of Lunar-based manufacturing and construction (LBMC), with a particular focus on the prospect of utilizing in-situ resources and additive manufacturing. The paper analyzes existing research on LBMC from various perspectives, including different manufacturing techniques and compositions, the potential of ISRU for LBMC, characterization of built parts and structures, the role of energy sources and efficiency, the impact of low-gravity and vacuum conditions, and the feasibility of using artificial intelligence, automation, and robotics. By synthesizing these findings, this review offers valuable insights into the challenges and opportunities that lie ahead for LBMC.

==> Sections/Abstract.tex <==
As humankind prepares to establish outposts and infrastructure on the Moon, the ability to manufacture parts and buildings on-site is crucial. While transporting raw materials from Earth can be costly and time-consuming, the use of ISRU (in-situ resource utilization) presents an attractive alternative. This review paper aims to provide a thorough examination of the current state and future potential of Lunar-based manufacturing, with a particular focus on the prospect of utilizing in-situ resources and additive manufacturing. 
This paper analyses the existing research on Lunar-based manufacturing from various perspectives, including the use of different manufacturing techniques, different compositions, the potential of ISRU for manufacturing and construction, the characterization of build parts and structures, the role of energy sources and efficiency, the impact of low-gravity and vacuum conditions, and the feasibility of using automation and robotics. By synthesizing these findings, this review offers valuable insights into the challenges and opportunities that lie ahead for Lunar-based manufacturing and construction (LBMC).
